Listening to Multi-talker Conversations: Modular and End-to-end Perspectives

Since the first speech recognition systems were built more than 30 years ago, improvement in voice technology has enabled applications such as smart assistants and automated customer support. However, conversation intelligence of the future requires recognizing free-flowing multi-party conversations, which is a crucial and challenging component that still remains unsolved. In this dissertation, we focus on this problem of speaker-attributed multi-talker speech recognition, and propose two perspectives which result from its probabilistic formulation. In the modular perspective, we build a pipeline of sub-tasks involving speaker diarization, target speaker extraction, and speech recognition. Our first contribution is a method to perform overlap-aware diarization by reformulating spectral clustering as a constrained optimization problem. We also describe an algorithm to ensemble diarization outputs, either to combine overlap-aware systems or to perform multi-channel diarization by late fusion. Once speaker segments are identified, we robustly extract single-speaker utterances from the mixture using a GPU-accelerated implementation of guided source separation, which allows us to use an off-the-shelf ASR system to obtain speaker-attributed transcripts. Since the modular approach suffers from error propagation, we propose an alternate "end-to-end" perspective on the problem. For this, we describe the Streaming Unmixing and Recognition Transducer (SURT). We show how to train SURT models efficiently by carefully designing the network architecture, objective functions, and mixture simulation techniques. Finally, we add an auxiliary speaker branch to enable joint prediction of speaker labels synchronized with the speech tokens. We demonstrate that training on synthetic mixtures and adapting with real data helps these models transfer well for streaming transcription of real meeting sessions.

==> committee/committee.tex <==
\chapter*{Thesis Committee}

\section*{}
\subsection*{Primary Readers}

\begin{singlespace}


\indent Sanjeev Khudanpur (Primary Advisor)\\
\indent \indent Associate Professor \\
\indent \indent Department of Electrical and Computer Engineering \\
\indent \indent  Johns Hopkins Whiting School of Engineering \\


\smallskip 

% \noindent First Lastname \\
% \indent \indent Assistant Professor\\
% \indent \indent Department of ChangeMe\\
% \indent \indent  Johns Hopkins Bloomberg School of Public Health \\

% \smallskip 

% \noindent First Lastname \\
% \indent \indent Assistant Professor\\
% \indent \indent Department of ChangeMe \\
% \indent \indent Johns Hopkins Bloomberg School of Public Health \\

% \smallskip


% \noindent First Lastname \\
% \indent \indent Associate Professor\\
% \indent \indent Affiliation1, and\\
% \indent \indent Department1 \& Department2 at\\
% \indent \indent Johns Hopkins Bloomberg School of Public Health \\


\end{singlespace}

\subsection*{Alternate Readers}

\begin{singlespace}


\indent First Lastname  \\
\indent \indent Professor\\
\indent \indent Department of ChangeMe\\
\indent \indent  Johns Hopkins Bloomberg School of Public Health \\

\noindent First Lastname  \\
\indent \indent Assistant Professor\\
\indent \indent Department of ChangeMe\\
\indent \indent  Johns Hopkins Bloomberg School of Public Health \\




\end{singlespace}
















